AI-assisted Optimization of the ECCE Tracking System at the Electron Ion Collider

The Electron-Ion Collider (EIC) is a cutting-edge accelerator facility that will study the nature of the "glue" that binds the building blocks of the visible matter in the universe. The proposed experiment will be realized at Brookhaven National Laboratory in approximately 10 years from now, with detector design and R&D currently ongoing. Notably, EIC is one of the first large-scale facilities to leverage Artificial Intelligence (AI) already starting from the design and R&D phases. The EIC Comprehensive Chromodynamics Experiment (ECCE) is a consortium that proposed a detector design based on a 1.5T solenoid. The EIC detector proposal review concluded that the ECCE design will serve as the reference design for an EIC detector. Herein we describe a comprehensive optimization of the ECCE tracker using AI. The work required a complex parametrization of the simulated detector system. Our approach dealt with an optimization problem in a multidimensional design space driven by multiple objectives that encode the detector performance, while satisfying several mechanical constraints. We describe our strategy and show results obtained for the ECCE tracking system. The AI-assisted design is agnostic to the simulation framework and can be extended to other sub-detectors or to a system of sub-detectors to further optimize the performance of the EIC detector.

==> authors/affiliations-test.tex <==
%
% Please fill in any missing information
%
%
% Example of the new format:
%
% \affiliation[]{organization={},
%	 addressline={},
%	 city={},
%	 postcode={},
%	 state={},
%	 country={}} 
%

\affiliation[AANL]{organization={A. Alikhanyan National Laboratory},
	 city={Yerevan},
	 country={Armenia}} 
 
\affiliation[AcademiaSinica]{organization={Institute of Physics, Academia Sinica},
	 city={Taipei},
	 country={Taiwan}} 
 
\affiliation[AUGIE]{organization={Augustana University},
	 addressline={},
	 city={Sioux Falls},
	 postcode={},
	 state={SD},
	 country={USA}} 
 
\affiliation[BNL]{organization={Brookhaven National Laboratory},
	 addressline={},
	 city={Upton},
	 postcode={11973},
	 state={NY},
	 country={USA}} 
 
\affiliation[BrunelUniversity]{organization={Brunel University London},
	 addressline={},
	 city={Uxbridge},
	 postcode={},
	 country={UK}} 
 
\affiliation[CanisiusCollege]{organization={Canisius College},
	 addressline={},
	 city={Buffalo},
	 postcode={},
	 state={NY},
	 country={USA}} 
 
\affiliation[CCNU]{organization={Central China Normal University},
	 city={Wuhan},
	 country={China}} 
 
\affiliation[Charles]{organization={Charles University},
	 city={Prague},
	 country={Czech Republic}} 
 
\affiliation[CIAE]{organization={China Institute of Atomic Energy, Fangshan},
	 city={Beijing},
	 country={China}} 
 
\affiliation[CNU]{organization={Christopher Newport University},
	 addressline={},
	 city={Newport News},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[Columbia]{organization={Columbia University},
	 addressline={},
	 city={New York},
	 postcode={},
	 state={NY},
	 country={USA}} 
 
\affiliation[CUA]{organization={Catholic University of America},
	 addressline={620 Michigan Ave.},
	 city={Washington DC},
	 postcode={20064},
	 country={USA}} 
 
\affiliation[CzechTechUniv]{organization={Czech Technical University},
	 addressline={},
	 city={Prague},
	 country={Czech Republic}} 
 
\affiliation[Duquesne]{organization={Duquesne University},
	 addressline={},
	 city={Pittsburgh},
	 postcode={},
	 state={PA},
	 country={USA}} 
 
\affiliation[Duke]{organization={Duke University},
	 addressline={},
	 city={},
	 postcode={},
	 state={NC},
	 country={USA}} 
 
\affiliation[FIU]{organization={Florida International University},
	 addressline={},
	 city={Miami},
	 postcode={},
	 state={FL},
	 country={USA}} 
 
\affiliation[GeorgiaState]{organization={Georgia State University},
	 addressline={},
	 city={Atlanta},
	 postcode={},
	 state={GA},
	 country={USA}} 
 
\affiliation[Glasgow]{organization={University of Glasgow},
	 addressline={},
	 city={Glasgow},
	 postcode={},
	 country={UK}} 
 
\affiliation[GSI]{organization={GSI Helmholtzzentrum fuer Schwerionenforschung},
	 addressline={},
	 city={Darmstadt},
	 postcode={},
	 country={Germany}} 
 
\affiliation[GWU]{organization={The George Washington University},
	 addressline={},
	 city={Washington, DC},
	 postcode={},
	 country={USA}} 
 
\affiliation[Hampton]{organization={Hampton University},
	 addressline={},
	 city={Hampton},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[HUJI]{organization={Hebrew University},
	 addressline={},
	 city={Jerusalem},
	 postcode={},
	 country={Isreal}} 
 
\affiliation[IMP]{organization={Chinese Academy of Sciences},
	 addressline={},
	 city={Lanzhou},
	 postcode={},
	 state={},
	 country={China}} 
 
\affiliation[IowaState]{organization={Iowa State University},
	 addressline={},
	 city={},
	 postcode={},
	 state={IA},
	 country={USA}} 
 
\affiliation[JazanUniversity]{organization={Jazan University},
	 city={Jazan},
	 country={Sadui Arabia}} 
 
\affiliation[JLab]{organization={Thomas Jefferson National Accelerator Facility},
	 addressline={12000 Jefferson Ave.},
	 city={Newport News},
	 postcode={24450},
	 state={VA},
	 country={USA}} 
 
\affiliation[JMU]{organization={James Madison University},
	 addressline={},
	 city={},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[KobeUniversity]{organization={Kobe University},
	 city={Kobe},
	 country={Japan}} 
 
\affiliation[Kyungpook]{organization={Kyungpook National University},
	 city={Daegu},
	 country={Republic of Korea}} 
 
\affiliation[LANL]{organization={Los Alamos National Laboratory},
	 addressline={},
	 city={},
	 postcode={},
	 state={NM},
	 country={USA}} 
 
\affiliation[LBNL]{organization={Lawrence Berkeley National Lab},
	 addressline={},
	 city={Berkeley},
	 postcode={},
	 state={},
	 country={USA}} 
 
\affiliation[LehighUniversity]{organization={Lehigh University},
	 addressline={},
	 city={Bethlehem},
	 postcode={},
	 state={PA},
	 country={USA}} 
 
\affiliation[LLNL]{organization={Lawrence Livermore National Laboratory},
	 addressline={},
	 city={Livermore},
	 postcode={},
	 state={CA},
	 country={USA}} 
 
\affiliation[MoreheadState]{organization={Morehead State University, Morehad, KY, USA},
	 addressline={},
	 city={Morehead},
	 postcode={},
	 state={KY},
	 country={USA}} 
 
\affiliation[MIT]{organization={Massachusetts Institute of Technology},
	 addressline={77 Massachusetts Ave.},
	 city={Cambridge},
	 postcode={02139},
	 state={MA},
	 country={USA}} 
 
\affiliation[MSU]{organization={Mississippi State University},
	 addressline={},
	 city={Mississippi State},
	 postcode={},
	 state={MS},
	 country={USA}} 
 
\affiliation[NCKU]{organization={ National Cheng Kung University, Tainan, Taiwan},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[NCU]{organization={National Central University},
	 city={Chungli},
	 country={Taiwan}} 
 
\affiliation[Nihon]{organization={Nihon University},
	 city={Tokyo},
	 country={Japan}} 
 
\affiliation[NMSU]{organization={New Mexico State University},
	 addressline={},
	 city={Las Cruces},
	 postcode={},
	 state={NM},
	 country={USA}} 
 
\affiliation[NRNUMEPhI]{organization={National Research Nuclear University MEPhI},
	 city={Moscow},
	 country={Russian Federation}} 
 
\affiliation[NRCN]{organization={Nuclear Research Center - Negev},
	 city={Beer-Sheva},
	 country={Isreal}} 
 
\affiliation[NTHU]{organization={National Tsing Hua University},
	 city={Hsinchu},
	 country={Taiwan}} 
 
\affiliation[NTU]{organization={National Taiwan University},
	 city={Taipei},
	 country={Taiwan}} 
 
\affiliation[ODU]{organization={Old Dominion University},
	 addressline={},
	 city={Norfolk},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[Ohio]{organization={Ohio University},
	 addressline={},
	 city={Athens},
	 postcode={},
	 state={OH},
	 country={USA}} 
 
\affiliation[ORNL]{organization={Oak Ridge National Laboratory},
	 addressline={PO Box 2008},
	 city={Oak Ridge},
	 postcode={37831},
	 state={TN},
	 country={USA}} 
 
\affiliation[PNNL]{organization={Pacific Northwest National Laboratory},
	 addressline={},
	 city={Richland},
	 postcode={},
	 state={WA},
	 country={USA}} 
 
\affiliation[Pusan]{organization={Pusan National Univeristy, Busan, Republic of Korea},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Rice]{organization={Rice University, Houston, TX, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[RIKEN]{organization={RIKEN Nishina Center, Wako, Saitama, Japan},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Rutgers]{organization={ The State University of New Jersey, Department of Physics and Astronomy, Piscataway, NJ, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
 
\affiliation[CFNS]{organization={Center for Frontiers in Nuclear Science},
	 addressline={Stony Brook Univeristy},
	 city={Stony Brook},
	 postcode={},
	 state={NY},
	 country={USA}} 
 
\affiliation[StonyBrook]{organization={ Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[RBRC]{organization={ RIKEN BNL Research Center, Brookhaven National Laboratory, , NY, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[SCNU]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Seoul]{organization={ Seoul National University, Seoul, Republic of Korea},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Sejong]{organization={ Sejong University, Seoul, Republic of Korea},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Shinshu]{organization={ Shinshu University, Matsumoto, Nagano, Japan},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Sungkyunkwan]{organization={ Sungkyunkwan University, Suwon, Republic of Korea},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[TAU]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Tokyo]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Tsinghua]{organization={ Tsinghua University, Beijing, China},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Tsukuba]{organization={ Tsukuba University of Technology, Tsukuba, Ibaraki, Japan.},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[CUBoulder]{organization={ University of Colorado Boulder, Boulder, CO, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UCAD]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UConn]{organization={ University of Connecticut, Storrs, CT, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UH]{organization={ University of Houston, Houston, TX, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UIUC]{organization={ University of Illinois, Urbana, IL, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UKansas]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UKY]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Ljubljana]{organization={ Faculty of Mathematics and Physics, University of Ljubljana, Ljubljana, Slovenia},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[NorthernGeorgia]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[NewHampshire]{organization={ University of New Hampshire, Durham, NH, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Oslo]{organization={ Department of Physics, University of Oslo, Norway},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Regina]{organization={ University of Regina, Regina, SK, Canada},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[USeoul]{organization={ University of Seoul, Seoul, Republic of Korea},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[USTC]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UTAustin]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UTsukuba]{organization={ University of Tsukuba, Tsukuba, Japan},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UTK]{organization={ University of Tennessee, Knoxville, TN, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UTSM]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UVA]{organization={ University of Virginia, Charlottesville, VA, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Vanderbilt]{organization={ Department of Physics and Astronomy, Vanderbilt University, Nashville, TN, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[VirginiaTech]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[VirginiaUnion]{organization={ Virginia Union University, Richmond, VA, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[WayneState]{organization={ Wayne State University, Detroit, MI, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[WI]{organization={ Department of Particle Physics and Astrophysics, Weizmann Institute of Science, Rehovot, Israel},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[WandM]{organization={ William and Mary, Williamsburg, VA, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Yamagata]{organization={ Faculty of Science, Yamagata University, Yamagata, Japan},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Yarmouk]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Yonsei]{organization={Yonsei University},
	 city={Seoul},
	 country={Republic of Korea}} 
 
\affiliation[York]{organization={University of York},
	 city={York},
	 country={UK}} 
 
\affiliation[Zagreb]{organization={University of Zagreb},
	 city={Zagreb},
	 country={Croatia}} 
 


==> authors/authorlist_new.tex <==
\author[MIT]{C.~Fanelli}
\author[Regina]{Z~Papandreou}
\author[Regina]{K.~Suresh}
\author[MoreheadState]{J.~K.~Adkins}
\author[RIKEN]{Y.~Akiba}
\author[UKansas]{A.~Albataineh}
\author[ODU]{M.~Amaryan}
\author[Oslo]{I.~C.~Arsene}
\author[Sungkyunkwan]{J.~Bae}
\author[UVA]{X.~Bai}
\author[Yonsei]{M.~Bashkanov}
\author[UH]{R.~Bellwied}
\author[Duquesne]{F.~Benmokhtar}
\author[CFNS,StonyBrook,RBRC]{J.~C.~Bernauer}
\author[ORNL]{F.~Bock}
\author[FIU]{W.~Boeglin}
\author[WI]{M.~Borysova}
\author[CNU]{E.~Brash}
\author[JLab]{P.~Brindza}
\author[GWU]{W.~J.~Briscoe}
\author[LANL]{M.~Brooks}
\author[ODU]{S.~Bueltmann}
\author[JazanUniversity]{M.~H.~S.~Bukhari}
\author[UKansas]{A.~Bylinkin}
\author[UConn]{R.~Capobianco}
\author[AcademiaSinica]{W.-C.~Chang}
\author[Sejong]{Y.~Cheon}
\author[CCNU]{K.~Chen}
\author[NTU]{K.-F.~Chen}
\author[NCU]{K.-Y.~Cheng}
\author[BNL]{M.~Chiu}
\author[UTsukuba]{T.~Chujo}
\author[BGU]{Z.~Citron}
\author[CFNS,StonyBrook]{E.~Cline}
\author[NRCN]{E.~Cohen}
\author[ORNL]{T.~Cormier}
\author[LANL]{Y.~Corrales~Morales}
\author[UVA]{C.~Cotton}
\author[UKY]{C.~Crawford}
\author[ORNL]{S.~Creekmore}
\author[JLab]{C.Cuevas}
\author[ORNL]{J.~Cunningham}
\author[BNL]{G.~David}
\author[LANL]{C.~T.~Dean}
\author[ORNL]{M.~Demarteau}
\author[UConn]{S.~Diehl}
\author[Yamagata]{N.~Doshita}
\author[IJCLabOrsay]{R.~Dupr\'{e}}
\author[LANL]{J.~M.~Durham}
\author[GSI]{R.~Dzhygadlo}
\author[ORNL]{R.~Ehlers}
\author[MSU]{L.~El~Fassi}
\author[UVA]{A.~Emmert}
\author[JLab]{R.~Ent}
\author[UKY]{R.~Fatemi}
\author[Yonsei]{S.~Fegan}
\author[Charles]{M.~Finger}
\author[Charles]{M.~Finger~Jr.}
\author[Ohio]{J.~Frantz}
\author[HUJI]{M.~Friedman}
\author[York]{I.~Friscic}
\author[UH]{D.~Gangadharan}
\author[Glasgow]{S.~Gardner}
\author[Glasgow]{K.~Gates}
\author[Rice]{F.~Geurts}
\author[Rutgers]{R.~Gilman}
\author[Glasgow]{D.~Glazier}
\author[ORNL]{E.~Glimos}
\author[RIKEN]{Y.~Goto}
\author[AUGIE]{N.~Grau}
\author[Vanderbilt]{S.~V.~Greene}
\author[IMP]{A.~Q.~Guo}
\author[FIU]{L.~Guo}
\author[Yarmouk]{S.~K.~Ha}
\author[BNL]{J.~Haggerty}
\author[UConn]{T.~Hayward}
\author[GeorgiaState]{X.~He}
\author[MIT]{O.~Hen}
\author[JLab]{D.~W.~Higinbotham}
\author[IJCLabOrsay]{M.~Hoballah}
\author[NTHU]{P.-h.~J.~Hsu}
\author[BNL]{J.~Huang}
\author[Regina]{G.~Huber}
\author[UH]{A.~Hutson}
\author[Yarmouk]{K.~Y.~Hwang}
\author[ODU]{C.~Hyde}
\author[Tsukuba]{M.~Inaba}
\author[Yamagata]{T.~Iwata}
\author[Kyungpook]{H.-S.~Jo}
\author[UConn]{K.~Joo}
\author[VirginiaUnion]{N.~Kalantarians}
\author[Shinshu]{K.~Kawade}
\author[Regina]{S.~Kay}
\author[UConn]{A.~Kim}
\author[Sungkyunkwan]{B.~Kim}
\author[Pusan]{C.~Kim}
\author[RIKEN]{M.~Kim}
\author[Pusan]{Y.~Kim}
\author[Sejong]{Y.~Kim}
\author[BNL]{E.~Kistenev}
\author[UConn]{V.~Klimenko}
\author[Seoul]{S.~H.~Ko}
\author[MIT]{I.~Korover}
\author[UKY]{W.~Korsch}
\author[UKansas]{G.~Krintiras}
\author[ODU]{S.~Kuhn}
\author[NCU]{C.-M.~Kuo}
\author[MIT]{T.~Kutz}
\author[IowaState]{J.~Lajoie}
\author[JLab]{D.~Lawrence}
\author[IowaState]{S.~Lebedev}
\author[Seoul]{J.~S.~H.~Lee}
\author[Kyungpook]{S.~W.~Lee}
\author[MIT]{Y.-J.~Lee}
\author[Rice]{W.~Li}
\author[CFNS,StonyBrook,WandM]{W.~Li}
\author[CIAE]{X.~Li}
\author[LANL]{X.~Li}
\author[IMP]{Y.~T.~Liang}
\author[Pusan]{S.~Lim}
\author[AcademiaSinica]{C.-h.~Lin}
\author[IMP]{D.~X.~Lin}
\author[LANL]{K.~Liu}
\author[LANL]{M.~X.~Liu}
\author[Glasgow]{K.~Livingston}
\author[UVA]{N.~Liyanage}
\author[WayneState]{W.~J.~Llope}
\author[ORNL]{C.~Loizides}
\author[NewHampshire]{E.~Long}
\author[NTU]{R.-S.~Lu}
\author[CIAE]{Z.~Lu}
\author[Yonsei]{W.~Lynch}
\author[IJCLabOrsay]{D.~Marchand}
\author[CzechTechUniv]{M.~Marcisovsky}
\author[FIU]{P.~Markowitz}
\author[LANL]{P.~McGaughey}
\author[Ljubljana]{M.~Mihovilovic}
\author[MIT]{R.~G.~Milner}
\author[WI]{A.~Milov}
\author[Yamagata]{Y.~Miyachi}
\author[CNU]{P.~Monaghan}
\author[Glasgow]{R.~Montgomery}
\author[BNL]{D.~Morrison}
\author[IJCLabOrsay]{C.~Munoz~Camacho}
\author[UKansas]{M.~Murray}
\author[LANL]{K.~Nagai}
\author[CUBoulder]{J.~Nagle}
\author[RIKEN]{I.~Nakagawa}
\author[UTK]{C.~Nattrass}
\author[JLab]{D.~Nguyen}
\author[IJCLabOrsay]{S.~Niccolai}
\author[BNL]{R.~Nouicer}
\author[RIKEN]{G.~Nukazuka}
\author[UVA]{M.~Nycz}
\author[NRNUMEPhI]{V.~A.~Okorokov}
\author[Regina]{S.~Ore\v{s}i\'{c}}
\author[ORNL]{J.D.~Osborn}
\author[LANL]{C.~O'Shaughnessy}
\author[NTU]{S.~Paganis}
\author[NMSU]{S.~Pate}
\author[IowaState]{M.~Patel}
\author[MIT]{C.~Paus}
\author[Glasgow]{G.~Penman}
\author[UIUC]{M.~G.~Perdekamp}
\author[CUBoulder]{D.~V.~Perepelitsa}
\author[LANL]{H.~Periera~da~Costa}
\author[GSI]{K.~Peters}
\author[CNU]{W.~Phelps}
\author[TAU]{E.~Piasetzky}
\author[BNL]{C.~Pinkenburg}
\author[Charles]{I.~Prochazka}
\author[LehighUniversity]{T.~Protzman}
\author[BNL]{M.~Purschke}
\author[WayneState]{J.~Putschke}
\author[MIT]{J.~R.~Pybus}
\author[JLab]{R.~Rajput-Ghoshal}
\author[ORNL]{J.~Rasson}
\author[FIU]{B.~Raue}
\author[ORNL]{K.~Read}
\author[Oslo]{K.~R\o{}ed}
\author[LehighUniversity]{R.~Reed}
\author[FIU]{J.~Reinhold}
\author[LANL]{E.~L.~Renner}
\author[UConn]{J.~Richards}
\author[UIUC]{C.~Riedl}
\author[BNL]{T.~Rinn}
\author[Ohio]{J.~Roche}
\author[MIT]{G.~M.~Roland}
\author[HUJI]{G.~Ron}
\author[IowaState]{M.~Rosati}
\author[UKansas]{C.~Royon}
\author[Pusan]{J.~Ryu}
\author[Rutgers]{S.~Salur}
\author[MIT]{N.~Santiesteban}
\author[UConn]{R.~Santos}
\author[GeorgiaState]{M.~Sarsour}
\author[ORNL]{J.~Schambach}
\author[GWU]{A.~Schmidt}
\author[ORNL]{N.~Schmidt}
\author[GSI]{C.~Schwarz}
\author[GSI]{J.~Schwiening}
\author[RIKEN]{R.~Seidl}
\author[UIUC]{A.~Sickles}
\author[UConn]{P.~Simmerling}
\author[Ljubljana]{S.~Sirca}
\author[GeorgiaState]{D.~Sharma}
\author[LANL]{Z.~Shi}
\author[Nihon]{T.-A.~Shibata}
\author[NCU]{C.-W.~Shih}
\author[RIKEN]{S.~Shimizu}
\author[UConn]{U.~Shrestha}
\author[NewHampshire]{K.~Slifer}
\author[LANL]{K.~Smith}
\author[LLNL]{R.~Soltz}
\author[LANL]{W.~Sondheim}
\author[CIAE]{J.~Song}
\author[Pusan]{J.~Song}
\author[GWU]{I.~I.~Strakovsky}
\author[BNL]{P.~Steinberg}
\author[WandM]{J.~Stevens}
\author[PNNL]{J.~Strube}
\author[CIAE]{P.~Sun}
\author[CCNU]{X.~Sun}
\author[NCU]{W.-C.~Tang}
\author[IowaState]{S.~Tapia~Araya}
\author[Vanderbilt]{S.~Tarafdar}
\author[BrunelUniversity]{L.~Teodorescu}
\author[UH]{A.~Timmins}
\author[CzechTechUniv]{L.~Tomasek}
\author[UConn]{N.~Trotta}
\author[Oslo]{T.~S.~Tveter}
\author[IowaState]{E.~Umaka}
\author[Regina]{A.~Usman}
\author[LANL]{H.~W.~van~Hecke}
\author[Vanderbilt]{J.~Velkovska}
\author[IJCLabOrsay]{E.~Voutier}
\author[IJCLabOrsay]{P.K.~Wang}
\author[UKansas]{Q.~Wang}
\author[CCNU]{Y.~Wang}
\author[Tsinghua]{Y.~Wang}
\author[Yonsei]{D.~P.~Watts}
\author[ODU]{L.~Weinstein}
\author[MIT]{M.~Williams}
\author[LANL]{C.-P.~Wong}
\author[PNNL]{L.~Wood}
\author[CanisiusCollege]{M.~H.~Wood}
\author[BNL]{C.~Woody}
\author[MIT]{B.~Wyslouch}
\author[Tsinghua]{Z.~Xiao}
\author[KobeUniversity]{Y.~Yamazaki}
\author[NCKU]{Y.~Yang}
\author[Tsinghua]{Z.~Ye}
\author[Yarmouk]{H.~D.~Yoo}
\author[LANL]{M.~Yurov}
\author[Yonsei]{N.~Zachariou}
\author[Columbia]{W.A.~Zajc}
\author[UVA]{J.~Zhang}
\author[Tsinghua]{Y.~Zhang}
\author[IMP]{Y.~X.~Zhao}
\author[UVA]{X.~Zheng}
\author[Tsinghua]{P.~Zhuang}

==> authors/authors-alphabetical-static.tex <==
\author[MoreheadState]{J.~K.~Adkins}
\author[RIKEN]{Y.~Akiba}
\author[UKansas]{A.~Albataineh}
\author[ODU]{M.~Amaryan}
\author[Oslo]{I.~C.~Arsene}
\author[Sungkyunkwan]{J.~Bae}
\author[UVA]{X.~Bai}
\author[Yonsei]{M.~Bashkanov}
\author[UH]{R.~Bellwied}
\author[Duquesne]{F.~Benmokhtar}
\author[CFNS,StonyBrook,RBRC]{J.~C.~Bernauer}
\author[ORNL]{F.~Bock}
\author[FIU]{W.~Boeglin}
\author[WI]{M.~Borysova}
\author[CNU]{E.~Brash}
\author[JLab]{P.~Brindza}
\author[GWU]{W.~J.~Briscoe}
\author[LANL]{M.~Brooks}
\author[ODU]{S.~Bueltmann}
\author[JazanUniversity]{M.~H.~S.~Bukhari}
\author[UKansas]{A.~Bylinkin}
\author[UConn]{R.~Capobianco}
\author[AcademiaSinica]{W.-C.~Chang}
\author[Sejong]{Y.~Cheon}
\author[CCNU]{K.~Chen}
\author[NTU]{K.-F.~Chen}
\author[NCU]{K.-Y.~Cheng}
\author[BNL]{M.~Chiu}
\author[UTsukuba]{T.~Chujo}
\author[BGU]{Z.~Citron}
\author[CFNS,StonyBrook]{E.~Cline}
\author[NRCN]{E.~Cohen}
\author[ORNL]{T.~Cormier}
\author[LANL]{Y.~Corrales~Morales}
\author[UVA]{C.~Cotton}
\author[UKY]{C.~Crawford}
\author[ORNL]{S.~Creekmore}
\author[JLab]{C.Cuevas}
\author[ORNL]{J.~Cunningham}
\author[BNL]{G.~David}
\author[LANL]{C.~T.~Dean}
\author[ORNL]{M.~Demarteau}
\author[UConn]{S.~Diehl}
\author[Yamagata]{N.~Doshita}
\author[IJCLabOrsay]{R.~Dupr\'{e}}
\author[LANL]{J.~M.~Durham}
\author[GSI]{R.~Dzhygadlo}
\author[ORNL]{R.~Ehlers}
\author[MSU]{L.~El~Fassi}
\author[UVA]{A.~Emmert}
\author[JLab]{R.~Ent}
\author[MIT]{C.~Fanelli}
\author[UKY]{R.~Fatemi}
\author[Yonsei]{S.~Fegan}
\author[Charles]{M.~Finger}
\author[Charles]{M.~Finger~Jr.}
\author[Ohio]{J.~Frantz}
\author[HUJI]{M.~Friedman}
\author[York]{I.~Friscic}
\author[UH]{D.~Gangadharan}
\author[Glasgow]{S.~Gardner}
\author[Glasgow]{K.~Gates}
\author[Rice]{F.~Geurts}
\author[Rutgers]{R.~Gilman}
\author[Glasgow]{D.~Glazier}
\author[ORNL]{E.~Glimos}
\author[RIKEN]{Y.~Goto}
\author[AUGIE]{N.~Grau}
\author[Vanderbilt]{S.~V.~Greene}
\author[IMP]{A.~Q.~Guo}
\author[FIU]{L.~Guo}
\author[Yarmouk]{S.~K.~Ha}
\author[BNL]{J.~Haggerty}
\author[UConn]{T.~Hayward}
\author[GeorgiaState]{X.~He}
\author[MIT]{O.~Hen}
\author[JLab]{D.W.~Higinbotham}
\author[IJCLabOrsay]{M.~Hoballah}
\author[NTHU]{P.-h.~J.~Hsu}
\author[BNL]{J.~Huang}
\author[Regina]{G.~Huber}
\author[UH]{A.~Hutson}
\author[Yarmouk]{K.~Y.~Hwang}
\author[ODU]{C.~Hyde}
\author[Tsukuba]{M.~Inaba}
\author[Yamagata]{T.~Iwata}
\author[Kyungpook]{H.-S.~Jo}
\author[UConn]{K.~Joo}
\author[VirginiaUnion]{N.~Kalantarians}
\author[Shinshu]{K.~Kawade}
\author[Regina]{S.~Kay}
\author[UConn]{A.~Kim}
\author[Sungkyunkwan]{B.~Kim}
\author[Pusan]{C.~Kim}
\author[RIKEN]{M.~Kim}
\author[Pusan]{Y.~Kim}
\author[Sejong]{Y.~Kim}
\author[BNL]{E.~Kistenev}
\author[UConn]{V.~Klimenko}
\author[Seoul]{S.~H.~Ko}
\author[MIT]{I.~Korover}
\author[UKY]{W.~Korsch}
\author[UKansas]{G.~Krintiras}
\author[ODU]{S.~Kuhn}
\author[NCU]{C.-M.~Kuo}
\author[MIT]{T.~Kutz}
\author[IowaState]{J.~Lajoie}
\author[JLab]{D.~Lawrence}
\author[IowaState]{S.~Lebedev}
\author[Seoul]{J.~S.~H.~Lee}
\author[Kyungpook]{S.~W.~Lee}
\author[MIT]{Y.-J.~Lee}
\author[Rice]{W.~Li}
\author[CFNS,StonyBrook,WandM]{W.~Li}
\author[CIAE]{X.~Li}
\author[LANL]{X.~Li}
\author[IMP]{Y.~T.~Liang}
\author[Pusan]{S.~Lim}
\author[AcademiaSinica]{C.-h.~Lin}
\author[IMP]{D.~X.~Lin}
\author[LANL]{K.~Liu}
\author[LANL]{M.~X.~Liu}
\author[Glasgow]{K.~Livingston}
\author[UVA]{N.~Liyanage}
\author[WayneState]{W.~J.~Llope}
\author[ORNL]{C.~Loizides}
\author[NewHampshire]{E.~Long}
\author[NTU]{R.-S.~Lu}
\author[CIAE]{Z.~Lu}
\author[Yonsei]{W.~Lynch}
\author[IJCLabOrsay]{D.~Marchand}
\author[CzechTechUniv]{M.~Marcisovsky}
\author[FIU]{P.~Markowitz}
\author[LANL]{P.~McGaughey}
\author[Ljubljana]{M.~Mihovilovic}
\author[MIT]{R.~G.~Milner}
\author[WI]{A.~Milov}
\author[Yamagata]{Y.~Miyachi}
\author[CNU]{P.~Monaghan}
\author[Glasgow]{R.~Montgomery}
\author[BNL]{D.~Morrison}
\author[IJCLabOrsay]{C.~Munoz~Camacho}
\author[UKansas]{M.~Murray}
\author[LANL]{K.~Nagai}
\author[CUBoulder]{J.~Nagle}
\author[RIKEN]{I.~Nakagawa}
\author[UTK]{C.~Nattrass}
\author[JLab]{D.~Nguyen}
\author[IJCLabOrsay]{S.~Niccolai}
\author[BNL]{R.~Nouicer}
\author[RIKEN]{G.~Nukazuka}
\author[UVA]{M.~Nycz}
\author[NRNUMEPhI]{V.~A.~Okorokov}
\author[Regina]{S.~Ore$\check{s}$i$\acute{c}$}
\author[ORNL]{J.~Osborn}
\author[LANL]{C.~O'Shaughnessy}
\author[NTU]{S.~Paganis}
\author[Regina]{Z~Papandreou}
\author[NMSU]{S.~Pate}
\author[IowaState]{M.~Patel}
\author[MIT]{C.~Paus}
\author[Glasgow]{G.~Penman}
\author[UIUC]{M.~G.~Perdekamp}
\author[CUBoulder]{D.~V.~Perepelitsa}
\author[LANL]{H.~Periera~da~Costa}
\author[GSI]{K.~Peters}
\author[CNU]{W.~Phelps}
\author[TAU]{E.~Piasetzky}
\author[BNL]{C.~Pinkenburg}
\author[Charles]{I.~Prochazka}
\author[LehighUniversity]{T.~Protzman}
\author[BNL]{M.~Purschke}
\author[WayneState]{J.~Putschke}
\author[MIT]{J.~R.~Pybus}
\author[JLab]{R.~Rajput-Ghoshal}
\author[ORNL]{J.~Rasson}
\author[FIU]{B.~Raue}
\author[ORNL]{K.~Read}
\author[Oslo]{K.~R$\o$ed}
\author[LehighUniversity]{R.~Reed}
\author[FIU]{J.~Reinhold}
\author[LANL]{E.~L.~Renner}
\author[UConn]{J.~Richards}
\author[UIUC]{C.~Riedl}
\author[BNL]{T.~Rinn}
\author[Ohio]{J.~Roche}
\author[MIT]{G.~M.~Roland}
\author[HUJI]{G.~Ron}
\author[IowaState]{M.~Rosati}
\author[UKansas]{C.~Royon}
\author[Pusan]{J.~Ryu}
\author[Rutgers]{S.~Salur}
\author[MIT]{N.~Santiesteban}
\author[UConn]{R.~Santos}
\author[GeorgiaState]{M.~Sarsour}
\author[ORNL]{J.~Schambach}
\author[GWU]{A.~Schmidt}
\author[ORNL]{N.~Schmidt}
\author[GSI]{C.~Schwarz}
\author[GSI]{J.~Schwiening}
\author[RIKEN]{R.~Seidl}
\author[UIUC]{A.~Sickles}
\author[UConn]{P.~Simmerling}
\author[Ljubljana]{S.~Sirca}
\author[GeorgiaState]{D.~Sharma}
\author[LANL]{Z.~Shi}
\author[Nihon]{T.-A.~Shibata}
\author[NCU]{C.-W.~Shih}
\author[RIKEN]{S.~Shimizu}
\author[UConn]{U.~Shrestha}
\author[NewHampshire]{K.~Slifer}
\author[LANL]{K.~Smith}
\author[LLNL]{R.~Soltz}
\author[LANL]{W.~Sondheim}
\author[CIAE]{J.~Song}
\author[Pusan]{J.~Song}
\author[GWU]{I.~I.~Strakovsky}
\author[BNL]{P.~Steinberg}
\author[WandM]{J.~Stevens}
\author[PNNL]{J.~Strube}
\author[CIAE]{P.~Sun}
\author[CCNU]{X.~Sun}
\author[Regina]{K.~Suresh}
\author[NCU]{W.-C.~Tang}
\author[IowaState]{S.~Tapia~Araya}
\author[Vanderbilt]{S.~Tarafdar}
\author[BrunelUniversity]{L.~Teodorescu}
\author[UH]{A.~Timmins}
\author[CzechTechUniv]{L.~Tomasek}
\author[UConn]{N.~Trotta}
\author[Oslo]{T.~S.~Tveter}
\author[IowaState]{E.~Umaka}
\author[Regina]{A.~Usman}
\author[LANL]{H.~W.~van~Hecke}
\author[Vanderbilt]{J.~Velkovska}
\author[IJCLabOrsay]{E.~Voutier}
\author[IJCLabOrsay]{P.K.~Wang}
\author[UKansas]{Q.~Wang}
\author[CCNU]{Y.~Wang}
\author[Tsinghua]{Y.~Wang}
\author[Yonsei]{D.~P.~Watts}
\author[ODU]{L.~Weinstein}
\author[MIT]{M.~Williams}
\author[LANL]{C.-P.~Wong}
\author[PNNL]{L.~Wood}
\author[CanisiusCollege]{M.~H.~Wood}
\author[BNL]{C.~Woody}
\author[MIT]{B.~Wyslouch}
\author[Tsinghua]{Z.~Xiao}
\author[KobeUniversity]{Y.~Yamazaki}
\author[NCKU]{Y.~Yang}
\author[Tsinghua]{Z.~Ye}
\author[Yarmouk]{H.~D.~Yoo}
\author[LANL]{M.~Yurov}
\author[Yonsei]{N.~Zachariou}
\author[Columbia]{W.A.~Zajc}
\author[UVA]{J.~Zhang}
\author[Tsinghua]{Y.~Zhang}
\author[IMP]{Y.~X.~Zhao}
\author[UVA]{X.~Zheng}
\author[Tsinghua]{P.~Zhuang}


==> authors/authors-alphabetical.tex <==
\author[MoreheadState]{J.~K.~Adkins}
\author[RIKEN]{Y.~Akiba}
\author[UKansas]{A.~Albataineh}
\author[ODU]{M.~Amaryan}
\author[Oslo]{I.~C.~Arsene}
\author[Sungkyunkwan]{J.~Bae}
\author[UVA]{X.~Bai}
\author[Yonsei]{M.~Bashkanov}
\author[UH]{R.~Bellwied}
\author[Duquesne]{F.~Benmokhtar}
\author[CFNS,StonyBrook,RBRC]{J.~C.~Bernauer}
\author[ORNL]{F.~Bock}
\author[FIU]{W.~Boeglin}
\author[WI]{M.~Borysova}
\author[CNU]{E.~Brash}
\author[JLab]{P.~Brindza}
\author[GWU]{W.~J.~Briscoe}
\author[LANL]{M.~Brooks}
\author[ODU]{S.~Bueltmann}
\author[JazanUniversity]{M.~H.~S.~Bukhari}
\author[UKansas]{A.~Bylinkin}
\author[UConn]{R.~Capobianco}
\author[AcademiaSinica]{W.-C.~Chang}
\author[Sejong]{Y.~Cheon}
\author[CCNU]{K.~Chen}
\author[NTU]{K.-F.~Chen}
\author[NCU]{K.-Y.~Cheng}
\author[BNL]{M.~Chiu}
\author[UTsukuba]{T.~Chujo}
\author[BGU]{Z.~Citron}
\author[CFNS,StonyBrook]{E.~Cline}
\author[NRCN]{E.~Cohen}
\author[ORNL]{T.~Cormier}
\author[LANL]{Y.~Corrales~Morales}
\author[UVA]{C.~Cotton}
\author[UKY]{C.~Crawford}
\author[ORNL]{S.~Creekmore}
\author[JLab]{C.Cuevas}
\author[ORNL]{J.~Cunningham}
\author[BNL]{G.~David}
\author[LANL]{C.~T.~Dean}
\author[ORNL]{M.~Demarteau}
\author[UConn]{S.~Diehl}
\author[Yamagata]{N.~Doshita}
\author[IJCLabOrsay]{R.~Dupr\'{e}}
\author[LANL]{J.~M.~Durham}
\author[GSI]{R.~Dzhygadlo}
\author[ORNL]{R.~Ehlers}
\author[MSU]{L.~El~Fassi}
\author[UVA]{A.~Emmert}
\author[JLab]{R.~Ent}
\author[MIT]{C.~Fanelli}
\author[UKY]{R.~Fatemi}
\author[Yonsei]{S.~Fegan}
\author[Charles]{M.~Finger}
\author[Charles]{M.~Finger~Jr.}
\author[Ohio]{J.~Frantz}
\author[HUJI]{M.~Friedman}
\author[York]{I.~Friscic}
\author[UH]{D.~Gangadharan}
\author[Glasgow]{S.~Gardner}
\author[Glasgow]{K.~Gates}
\author[Rice]{F.~Geurts}
\author[Rutgers]{R.~Gilman}
\author[Glasgow]{D.~Glazier}
\author[ORNL]{E.~Glimos}
\author[RIKEN]{Y.~Goto}
\author[AUGIE]{N.~Grau}
\author[Vanderbilt]{S.~V.~Greene}
\author[IMP]{A.~Q.~Guo}
\author[FIU]{L.~Guo}
\author[Yarmouk]{S.~K.~Ha}
\author[BNL]{J.~Haggerty}
\author[UConn]{T.~Hayward}
\author[GeorgiaState]{X.~He}
\author[MIT]{O.~Hen}
\author[JLab]{D.~W.~Higinbotham}
\author[IJCLabOrsay]{M.~Hoballah}
\author[NTHU]{P.-h.~J.~Hsu}
\author[BNL]{J.~Huang}
\author[Regina]{G.~Huber}
\author[UH]{A.~Hutson}
\author[Yarmouk]{K.~Y.~Hwang}
\author[ODU]{C.~Hyde}
\author[Tsukuba]{M.~Inaba}
\author[Yamagata]{T.~Iwata}
\author[Kyungpook]{H.-S.~Jo}
\author[UConn]{K.~Joo}
\author[VirginiaUnion]{N.~Kalantarians}
\author[Shinshu]{K.~Kawade}
\author[Regina]{S.~Kay}
\author[UConn]{A.~Kim}
\author[Sungkyunkwan]{B.~Kim}
\author[Pusan]{C.~Kim}
\author[RIKEN]{M.~Kim}
\author[Pusan]{Y.~Kim}
\author[Sejong]{Y.~Kim}
\author[BNL]{E.~Kistenev}
\author[UConn]{V.~Klimenko}
\author[Seoul]{S.~H.~Ko}
\author[MIT]{I.~Korover}
\author[UKY]{W.~Korsch}
\author[UKansas]{G.~Krintiras}
\author[ODU]{S.~Kuhn}
\author[NCU]{C.-M.~Kuo}
\author[MIT]{T.~Kutz}
\author[IowaState]{J.~Lajoie}
\author[JLab]{D.~Lawrence}
\author[IowaState]{S.~Lebedev}
\author[Seoul]{J.~S.~H.~Lee}
\author[Kyungpook]{S.~W.~Lee}
\author[MIT]{Y.-J.~Lee}
\author[Rice]{W.~Li}
\author[CFNS,StonyBrook,WandM]{W.~Li}
\author[CIAE]{X.~Li}
\author[LANL]{X.~Li}
\author[IMP]{Y.~T.~Liang}
\author[Pusan]{S.~Lim}
\author[AcademiaSinica]{C.-h.~Lin}
\author[IMP]{D.~X.~Lin}
\author[LANL]{K.~Liu}
\author[LANL]{M.~X.~Liu}
\author[Glasgow]{K.~Livingston}
\author[UVA]{N.~Liyanage}
\author[WayneState]{W.~J.~Llope}
\author[ORNL]{C.~Loizides}
\author[NewHampshire]{E.~Long}
\author[NTU]{R.-S.~Lu}
\author[CIAE]{Z.~Lu}
\author[Yonsei]{W.~Lynch}
\author[IJCLabOrsay]{D.~Marchand}
\author[CzechTechUniv]{M.~Marcisovsky}
\author[FIU]{P.~Markowitz}
\author[LANL]{P.~McGaughey}
\author[Ljubljana]{M.~Mihovilovic}
\author[MIT]{R.~G.~Milner}
\author[WI]{A.~Milov}
\author[Yamagata]{Y.~Miyachi}
\author[CNU]{P.~Monaghan}
\author[Glasgow]{R.~Montgomery}
\author[BNL]{D.~Morrison}
\author[IJCLabOrsay]{C.~Munoz~Camacho}
\author[UKansas]{M.~Murray}
\author[LANL]{K.~Nagai}
\author[CUBoulder]{J.~Nagle}
\author[RIKEN]{I.~Nakagawa}
\author[UTK]{C.~Nattrass}
\author[JLab]{D.~Nguyen}
\author[IJCLabOrsay]{S.~Niccolai}
\author[BNL]{R.~Nouicer}
\author[RIKEN]{G.~Nukazuka}
\author[UVA]{M.~Nycz}
\author[NRNUMEPhI]{V.~A.~Okorokov}
\author[Regina]{S.~Ore\v{s}i\'{c}}
\author[ORNL]{J.D.~Osborn}
\author[LANL]{C.~O'Shaughnessy}
\author[NTU]{S.~Paganis}
\author[Regina]{Z~Papandreou}
\author[NMSU]{S.~Pate}
\author[IowaState]{M.~Patel}
\author[MIT]{C.~Paus}
\author[Glasgow]{G.~Penman}
\author[UIUC]{M.~G.~Perdekamp}
\author[CUBoulder]{D.~V.~Perepelitsa}
\author[LANL]{H.~Periera~da~Costa}
\author[GSI]{K.~Peters}
\author[CNU]{W.~Phelps}
\author[TAU]{E.~Piasetzky}
\author[BNL]{C.~Pinkenburg}
\author[Charles]{I.~Prochazka}
\author[LehighUniversity]{T.~Protzman}
\author[BNL]{M.~Purschke}
\author[WayneState]{J.~Putschke}
\author[MIT]{J.~R.~Pybus}
\author[JLab]{R.~Rajput-Ghoshal}
\author[ORNL]{J.~Rasson}
\author[FIU]{B.~Raue}
\author[ORNL]{K.~Read}
\author[Oslo]{K.~R\o{}ed}
\author[LehighUniversity]{R.~Reed}
\author[FIU]{J.~Reinhold}
\author[LANL]{E.~L.~Renner}
\author[UConn]{J.~Richards}
\author[UIUC]{C.~Riedl}
\author[BNL]{T.~Rinn}
\author[Ohio]{J.~Roche}
\author[MIT]{G.~M.~Roland}
\author[HUJI]{G.~Ron}
\author[IowaState]{M.~Rosati}
\author[UKansas]{C.~Royon}
\author[Pusan]{J.~Ryu}
\author[Rutgers]{S.~Salur}
\author[MIT]{N.~Santiesteban}
\author[UConn]{R.~Santos}
\author[GeorgiaState]{M.~Sarsour}
\author[ORNL]{J.~Schambach}
\author[GWU]{A.~Schmidt}
\author[ORNL]{N.~Schmidt}
\author[GSI]{C.~Schwarz}
\author[GSI]{J.~Schwiening}
\author[RIKEN]{R.~Seidl}
\author[UIUC]{A.~Sickles}
\author[UConn]{P.~Simmerling}
\author[Ljubljana]{S.~Sirca}
\author[GeorgiaState]{D.~Sharma}
\author[LANL]{Z.~Shi}
\author[Nihon]{T.-A.~Shibata}
\author[NCU]{C.-W.~Shih}
\author[RIKEN]{S.~Shimizu}
\author[UConn]{U.~Shrestha}
\author[NewHampshire]{K.~Slifer}
\author[LANL]{K.~Smith}
\author[LLNL]{R.~Soltz}
\author[LANL]{W.~Sondheim}
\author[CIAE]{J.~Song}
\author[Pusan]{J.~Song}
\author[GWU]{I.~I.~Strakovsky}
\author[BNL]{P.~Steinberg}
\author[WandM]{J.~Stevens}
\author[PNNL]{J.~Strube}
\author[CIAE]{P.~Sun}
\author[CCNU]{X.~Sun}
\author[Regina]{K.~Suresh}
\author[NCU]{W.-C.~Tang}
\author[IowaState]{S.~Tapia~Araya}
\author[Vanderbilt]{S.~Tarafdar}
\author[BrunelUniversity]{L.~Teodorescu}
\author[UH]{A.~Timmins}
\author[CzechTechUniv]{L.~Tomasek}
\author[UConn]{N.~Trotta}
\author[Oslo]{T.~S.~Tveter}
\author[IowaState]{E.~Umaka}
\author[Regina]{A.~Usman}
\author[LANL]{H.~W.~van~Hecke}
\author[Vanderbilt]{J.~Velkovska}
\author[IJCLabOrsay]{E.~Voutier}
\author[IJCLabOrsay]{P.K.~Wang}
\author[UKansas]{Q.~Wang}
\author[CCNU]{Y.~Wang}
\author[Tsinghua]{Y.~Wang}
\author[Yonsei]{D.~P.~Watts}
\author[ODU]{L.~Weinstein}
\author[MIT]{M.~Williams}
\author[LANL]{C.-P.~Wong}
\author[PNNL]{L.~Wood}
\author[CanisiusCollege]{M.~H.~Wood}
\author[BNL]{C.~Woody}
\author[MIT]{B.~Wyslouch}
\author[Tsinghua]{Z.~Xiao}
\author[KobeUniversity]{Y.~Yamazaki}
\author[NCKU]{Y.~Yang}
\author[Tsinghua]{Z.~Ye}
\author[Yarmouk]{H.~D.~Yoo}
\author[LANL]{M.~Yurov}
\author[Yonsei]{N.~Zachariou}
\author[Columbia]{W.A.~Zajc}
\author[UVA]{J.~Zhang}
\author[Tsinghua]{Y.~Zhang}
\author[IMP]{Y.~X.~Zhao}
\author[UVA]{X.~Zheng}
\author[Tsinghua]{P.~Zhuang}


==> sections/backup.tex <==
\begin{comment}
\begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/dRICH_BO_scheme.png}
    \caption{
    Bayesian optimization framework for the optimization of the dual-RICH. N detector design points are created in parallel and passed to the BO which uses Gaussian processes, which collects the points, updates the surrogate model (a 2D visualization is shown in the bottom right corner considering all pairs of design parameters). A cheap acquisition function suggests a new set of design points to query at the next iteration. Convergence criteria are implemented on both the design space and on the objective (in this case, the $\pi$/K separation power of the dual-RICH) and early stopping is activated when convergence is observed in both spaces. Figure taken from \cite{fanelli_jluo2021}. More details can be found in \cite{cisbani2020ai}.   
    }
    \label{fig:dRICH_BO_scheme}
\end{figure}
\end{comment}

%identify the solutions that can approximate the sought performance in the functional space (see, \textit{e.g.}, \cite{sanchez2018inverse}). 




%Leveraging on the expertise internal to the ECCE proto-collaboration --- see, \textit{e.g.}, the optimization of imaging Cherenkov detectors with AI-based techniques \cite{cisbani2020ai} with a workflow described in Fig. \ref{fig:dRICH_BO_scheme} --- 



%The first parallelized, automated and self-consistent AI-supported strategy for detector optimization has been demonstrated for the dual-RICH in a work led by  \cite{cisbani2020ai}.

%leveraging Bayesian optimization (BO) \cite{snoek2012practical}. 
%A workflow of this framework is shown in Fig.~\ref{fig:dRICH_BO_scheme}, where more details can be found. 

 % see Fig. \ref{fig:pipeline_workflow} (bottom).

\begin{comment}
 \begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/interplay_groups.png}
    \caption{
    A workflow describing the iterative process of detector design. AI assisted this process, provided insights and helped capturing hidden correlations among the design parameters. 
    This has been used during the detector technology choice to steer the design. At a given instant in time, N alternative candidate configurations are studied. For each we create an optimization pipeline, which results in a Pareto front of solutions. This new information helps the proto-collaboration steering the design: some configurations are rejected, while alternative ones (also dubbed `new references') are identified to potentially improve the design. New optimization pipelines (we typically handled a maximum of 4-5 pipelines each time) are defined based on these alternatives and the process is iterated. 
    The fundamental interplay between the ECCE Teams working on Physics(PWG), Detector(DWG) and Computing(CWG) is clearly propelled by AI during the design process. 
}
    \label{fig:pipeline_workflow}
\end{figure}
\end{comment}



%----------------------- slanted figures ----------------------%


\begin{comment}
\begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/NonProjectiveGeom_Detailed_Slanted.pdf}
    \caption{\textbf{The ECCE tracking and PID system during Phase-I optimisation:} This is one of the studied configurations. Multiple pipelines corresponding to different combinations of technology for the barrels and the disks have been studied. Since the arrangement is symmetric, optimisations are done in $\eta$ corresponding only to the barrel region and the forward-region. The labels given in red are considered for optimisation, and the labels in blue are fixed in their locations. The geometry displays a non-projective design of the support structure.}
    \label{fig:Phase-I_ECCEDetector}
\end{figure}
\end{comment}


\begin{comment}
\begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ProjectiveGeom_Detailed_Slanted.pdf}
    \caption{\textbf{Tracking and PID systems in the ongoing R\&D projective design:} Starting from the IP, angle of the conical support structure ($\theta$) which defines the angle of the projective geometry. Followed by 3 vertex barrel layers (ITS3 technology), followed by 2 sagitta layers (ITS3 techonology), 2 $\mu$Rwell layers, ACLGAD based CTTL Time Of Flight (TOF) detector, DIRC (for PID) detector and finally another layer of $\mu$Rwell. In the electron-going direction there are 4 EST disks (silicon disks) followed by MPGD, mRICH (PID) detector and ACLGAD based ETTL TOF disk. In the hadron-going direction there are 5 FST disks (silicon disks) followed by a layer of ACLGAD based FTTL TOF disk, the dRICH (PID) detector and finally a layer of MPGD disk. The labels in red are the detector systems that are considered for optimisation. The labels in blue are the detector systems that are not free parameters and are not optimised during the optimisation. Some of the detectors parameters given in blue are parameterised such that they change as the design varies The Tracking support cone comprises copper and plastic insulation along with carbon fiber and the cooling system (water). The support cone is relatively thick up to 1cm for over the optimisation.  %\cris{sentence not clear} The labels in blue are the detector systems that either have their dimensions fixed or is parameterised during the optimisation as they are not free parameter
    }
    \label{fig:ECCE_TrackingPID_Detailed}
\end{figure}
\end{comment}




\begin{table}[bh!]
   
    \centering
    \begin{tabular}{|M{3.cm} | M{1.5cm}| M{2.0cm}|}
        \hline
        \textbf{description} & \textbf{symbol} & \textbf{value} \\ 
        \hline
        \hline
        \small{population size} & N & 100 \\
        \small{\# objectives}   & M & 3(4)\\ 
        \small{offspring} & O & 30(50)\\
        \small{design size} & D & 4(11) \\
        \small{\# calls (tot. budget)} & $-$ & 50(200)\\
        \small{\# cores} & $-$ & \small{same as offspring} \\
        \small{\# charged $\pi$ tracks} & N$_{\textup{trk}}$ & 80k\\
        \small{\# bins in $\eta$} & N$_{\eta}$ & 3 (5)\\
        \small{\# bins in P} & N$_{\textup{P}}$ & 10 (15) \\
        \hline
    \end{tabular}
    \caption{ Summary of the hyperparameters used for the non-projective tracker design. Symbols used throughout the document to describe these quantities are also reported to facilitate the reader. %For each parameter, in parentheses one can find the maximum value that has been explored. 
     Values in parentheses are the largest ones utilized in the optimization pipelines. The total number of design vary between Phase-I and Phase-II. Phase-II optimization involved accommodating realistic support structure and therefore constraining the overall design space. Checkpoints are created allowing to take a snapshot of the optimization while ongoing. A survey of the detector performance is created after each call. At each call an offspring of 30 or 50 new design points has been created through a genetic algorithm. A two-level parallelization is implemented as explained in Sec.~\ref{subsec:computing}. %The framework ran on the JLab computing farm which currently host nodes with a maximum number of 128 cores.
     \cris{merge with Table~\ref{tab:Complexity_Proj}.}
     \label{tab:Complexity_NonProj}
    }
    
\end{table}



\begin{table}[h!]
    \centering
    \begin{tabular}{|M{3.cm} | M{1.5cm}| M{2.0cm}|}
        \hline
        \textbf{description} & \textbf{symbol} & \textbf{value} \\ 
        \hline
        \hline
        \small{population size} & N & 100 \\
        \small{\# objectives}   & M & 3(4)\\ 
        \small{offspring} & O & 30(50)\\
        \small{design size} & D & 11(16) \\
        \small{\# calls (tot. budget)} & $-$ & 200\\
        \small{\# cores} & $-$ & \small{same as offspring} \\
        \small{\# charged $\pi$ tracks} & N$_{\textup{trk}}$ & 120k\\
        \small{\# bins in $\eta$} & N$_{\eta}$ & 5 \\
        \small{\# bins in P} & N$_{\textup{P}}$ & 10 \\
        \hline
    \end{tabular}
    \caption{Summary of the hyperparameters utilized for the projective design. Values in parentheses are the largest ones utilized in other optimization pipelines. Checkpoints are created allowing to take a snapshot of the optimization while ongoing. A survey of the detector performance is created after each call. At each call an offspring of new design points is created through a genetic algorithm. %A two-level parallelization is implemented as explained in the text. The framework ran on the JLab computing farm which currently host nodes with a maximum number of 128 cores.
    }
    \label{tab:Complexity_Proj}
\end{table}
%



\begin{table}[!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{M{2.5cm}|M{3.cm}|M{3.cm}|M{3.5cm}}
        \hline
        & \textbf{design pars} &  \textbf{objectives} &  \textbf{constraints} \\
        \hline
        \hline
           \textbf{\#} &  4(11) &  3 (4) &  4(5) \\
        \hline
           \textbf{description} & \small{(Phase-I symmetric design) 5 disks $z$-location (hadron beam) and 6 barrel layers radii; (Phase-II asymmertic design) 3 disks $z$ location (endcap region) 1 barrel layer} & \small{momentum resolution; angular resolution; Kalman filter efficiency; (pointing resolution)}
           & \small{(i) inner 2$^{nd}$ vtx barrel radius $\leq$ 15 cm; (ii) outermost barrel radius $<$ 51 cm; (iii) outermost $z$ disk $<$ 125 cm; (iv) 4$^{th}$ barrel radius $\leq$ 45 cm; (v) Minimum distance between any 2 layers $>=$ 1 cms (Additional constraints for Phase-II)} \\
        \hline
        \hline
    \end{tabular}
    }
    \caption{Dimensionality of the non-projective design and objective space. Following Eq.~\eqref{eq:moo}, constraints are also included. For each category, a description has been added.  Values in parentheses are the largest ones utilized in the optimization pipelines.
    The Phase-II optimization had less number of parameters to optimize due to the fixed support cone structure.  Notice that two additional constraints are implicitly taken into account, that is: (i) the inner radii of the disks in the endcap and the inner vertex layer in the barrel have to be compatible with the beam envelope dimensions; (ii) the barrel layers lengths and the outer radii of the disks have to be compatible with an Al-shell support structure provided by the LBNL design \cite{arrington2021eic}. Conditions (i) and (ii) are provided by internal parametrization and reflected in the Geant4 design. Potential overlaps among modules are checked before and during the optimization.}
    \label{tab:Problem_NonProj}
\end{table}


\begin{comment}
\begin{table}[!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{M{2.5cm}|M{3.cm}|M{3.cm}|M{3.5cm}}
    %\begin{tabular}{c|c|c|c}
        \hline
        & \textbf{design pars} &  \textbf{objectives} &  \textbf{constraints} \\
        \hline
        \hline
           \textbf{\#} &  11 (16) &  4 &  3 (5)\\
        \hline
           \textbf{description} & \small{(symmetric design) Angle Tracking Support ($\theta$), 2 TTL $z$-location, 2 MPGD $z$-location, 1 uRwell-1 Radius, 5 EST/FST disks; (asymmetric design) total of 16 params} & \small{momentum resolution; angular resolution; Kalman filter efficiency; angular resolution at dRICH; (pointing resolution)}
           & \small{(i) FST/EST Disks $(R_{Max}-R_{Min})\%(30.0 \ mm)=0$; (ii) FST/EST Disks $(R_{Max}-R_{Min})\%(17.8 \ mm)=0$; (iii) FST/EST $z_{n+1} - z_{n} \geq 10$; (iv) Length of vertex support structure $\leq$ 30 cms; (v) distance between any 2 $\mu$Rwell barrel layers have to be atleast 5 cms; } 
           %\cris{larger! It was smaller...} 
           \\
        \hline
        \hline
    \end{tabular}
    }
    \caption{Dimensionality of the problem in the projective design and objective space. Following Eq.~\eqref{eq:moo}, constraints are also included. For each category, a description has been added. Number in parentheses are for optimizations pipelines utilizing an asymmetric design with both the cone angle in e-going and h-going side to vary. However, the set up with different angles in e-going and h-going directions was not preferred as it would be difficult to realise such a design.
    }
    \label{tab:Problem_Proj}
\end{table}
\end{comment}


\begin{comment}
\begin{table}[!]
    \centering
    \begin{tabular}{|M{1.5cm}|M{4.5cm}|M{4.5cm}|}
        \hline
        $\#$ & Objectives & Ratio \\
        \hline
        \hline
        1 & Momentum Resolution Eq.~\eqref{eq:obj_definition} & Eq.~\eqref{eq:objectives_reso}\\
        \hline
        2 & Angular Resolution ($d\theta$) Eq.~\eqref{eq:obj_definition} & Eq.~\eqref{eq:objectives_reso}\\
        \hline
        3 & Kalman Filter InEfficiency & Ratio: Eq.~\eqref{eq:objective_KF} \\
        \hline
        4 & Angular Resolution $@$ dRICH (PID) Eq.~\eqref{eq:obj_definition_PID} & Ratio Equation: Eq.~\eqref{eq:Objectives_Reso} \\
        \hline
    \end{tabular}
    \caption{
    \cris{add caption; this table is for the projective case.};
    %The table summarises constraints on the design problem. Mainly the constraints are on the FST/EST disks are made by tiling up the MAPS pixels. The pixels will be made are of fixed dimensions. Soft constraints are constraints that can be violated but the MOO will evolve to minimally violate the constraints. Also, minor adjustments on tiling up the pixels can be done post hoc optimization such that the Detector geometry is realisable. Strong constraints penalises the MOO with high penalities since these constraints cannot be violated.
    }
    \label{tab:Objectives_proj}
\end{table}
\end{comment}



\begin{comment}
\begin{figure*}[!]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_1.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_2.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_3.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_4.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_5.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_6.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_7.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_8.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_9.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_10.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_11.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_12.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_13.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_14.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_15.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_16.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_17.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_18.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_19.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_20.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_21.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_22.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_23.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_24.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_25.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_26.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_27.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_28.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_29.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_30.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_31.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_32.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_33.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_34.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_35.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_36.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_37.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_38.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_39.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_40.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_41.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_42.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_43.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_44.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_45.pdf}}
    {}
\\
\hline
\end{tabular}
\caption{The resolutions are fitted in bins of momentum and pseudo-rapidity. The figures displays the example of the momentum resolution, which is calculated in multiple bins in the region 0~$\leq$P$\leq$~30~GeV/c and 0~$\leq \eta \leq$~3.5. These studies are extended to the e-going direction with negative values of $\eta$.
\label{fig:fit_results}
}
\end{figure*}
\end{comment}



%----------------------- all tables go here -------------------%
% non-projective 
% projective 

Tables \ref{tab:Complexity_NonProj} and \ref{tab:Problem_NonProj} summarize the overall implementation of different pipelines for the non-projective design corresponding to both Phase-I and Phase-II optimizations. 

Tables \ref{tab:Complexity_Proj} and \ref{tab:Problem_Proj} summarize the overall implementation of different pipelines during Phase II for the projective design. 

Table \ref{tab:Parameter_Range_Proj} reports in particular the range of parameters utilized in the projective design.  

%Table \ref{tab:constraints} is a table summarizing the constraints utilized in the MOO problem. 



\cris{Merging of tables here.}

%Additionally \ref{tab:constraints} provide constraints for the optimization of Phase-II non Projective optimizations. Therefore, Phase-II non Projective Optmisation was highly constrained.


\cris{Checkpoints are created allowing to take a snapshot of the optimization while ongoing. 
%
A survey of the detector performance is created after each call. 
%
At each call an offspring of 30  new design points has been created through a genetic algorithm. A two-level parallelization is implemented as explained in Sec.~\ref{subsec:computing}.
}


\begin{comment}
%-------------------------------------------
\paragraph{Design Performance (Phase I):} 
%
Performance is shown in terms of the objective functions utilized during the optimization process. 
After the optimization, these functions are shown as a function of the phase-space (P,$\eta$). \cris{utilize P uniformly in the text}.

One particular solution from the Pareto front is taken here as an example. Fig.~\ref{fig:FrozenAnalysis_dpp} shows the momentum resolution corresponding to the baseline design of one of the pipelines from Phase-I optimization. This solution in the Pareto front shows about 20 $\%$ improvement in central and extreme forward regions. 
A similar plot in Fig.~\ref{fig:FrozenAnalysis_dth} shows the angular resolution ($d\theta$) corresponding to the baseline design, where an improvement is seen at large values of $\eta$.
The other objective is the Kalman filter inefficiency which has been minimized together with the other two objectives. 
Fig.~\ref{fig:FrozenAnalysis_KFInEff} shows the resulting KF efficiency, where it can be seen a substantial improvement with AI in the overall region $\eta$ $>$ 1.

\begin{figure}[!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dp_p_p_eta_0 - 1.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dp_p_p_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dp_p_p_eta_2.5 - 3.5.pdf}}
    {}

\\
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dp_p_p_eta_0 - 1.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dp_p_p_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dp_p_p_eta_2.5 - 3.5.pdf}}
    {}
\\
\hline
\end{tabular}
\caption{Momentum resolution corresponding to the Baseline design of one of the pipelines from Phase-I optimization. From Left to right in top row corresponds to momentum resolutions in various bins in eta. The objective calculated during optimization is based on 3 bins in $\eta$ and the optimization assumes a symmetric arrangement of detectors in the endcap region. Therefore, optimization was carried out only in the forward region ($\eta > 0$). The bottom row shows the ratio of the optimal solution to that of the baseline (reference) design performance. We see about 20 $\%$ improvement in central and extreme forward regions. Therefore, the optimal solution outperforms in all the bins in $\eta$.}
\label{fig:FrozenAnalysis_dpp}
\end{figure}


\begin{figure}[!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dth_th_p_eta_0 - 1.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dth_th_p_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dth_th_p_eta_2.5 - 3.5.pdf}}
    {}

\\
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dth_th_p_eta_0 - 1.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dth_th_p_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dth_th_p_eta_2.5 - 3.5.pdf}}
    {}
\\
\hline
\end{tabular}
\caption{Angular resolution ($d\theta$) corresponding to the Baseline design of one of the pipelines from Phase-I optimization. From Left to right in top row corresponds to momentum resolutions in various bins in eta. The objective calculated during optimization is based on 3 bins in $\eta$ and the optimization assumes a symmetric arrangement of detectors in the endcap region. Therefore, optimization was carried out only in the forward region ($\eta > 0$). The bottom row shows the ratio of the optimal solution to that of the baseline (reference) design performance. We see an improvement in $2.5 < |\eta| < 3.5$ and performs similar in other bins.}
\label{fig:FrozenAnalysis_dth}
\end{figure}


\begin{figure}[!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_KF_InEfficiency_eta_0 - 1.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_KF_InEfficiency_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_KF_InEfficiency_eta_2.5 - 3.5.pdf}}
    {}

\\
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_KF_InEfficiency_eta_0 - 1.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_KF_InEfficiency_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_KF_InEfficiency_eta_2.5 - 3.5.pdf}}
    {}
\\
\hline
\end{tabular}
\caption{Kalman Filter efficiency corresponding to the Baseline design of one of the pipelines from Phase-I optimization. From Left to right in top row corresponds to momentum resolutions in various bins in eta. The objective calculated during optimization is based on 3 bins in $\eta$ and the optimization assumes a symmetric arrangement of detectors in the endcap region. Therefore, optimization was carried out only in the forward region ($\eta > 0$). The bottom row shows the ratio of the optimal solution to that of the baseline (reference) design performance. We see an improvement in mid region $ 1.0 < \eta < 2.5 $ and $2.5 < |\eta| < 3.5$ and performs similar in other bins.
\cris{Ratios are for the inefficiency. THIS IS A PLACEHOLDER}.
}
\label{fig:FrozenAnalysis_KFInEff}
\end{figure}
\end{comment}




%%%% Start of Phase -I results %%%%%%
\begin{comment}
\paragraph{Design Performance in Phase I}

Phase-I optimization as mentioned earlier, corresponds to a set of optimizations that were done on a symmetric arrange of disks in both electron-going and hadron-going directions. 
Some of the detectors like the PID and TOF detectors were modelled using fast simulation. The optimization did not include the  cone structure and hence the active dead material interaction was not minimized in the optimization process. There were 4 combinations of technologies (pipelines) that were proposed for the inner barrel tracking system. Each combination was explored and optimized using the developed framework. Fig.~\ref{fig:Phase-I_Pipelines} shows the momentum resolution of the explored pipelines and the corresponding optimized performance. 

\begin{figure*}[!]
\centering
\begin{tabular}{c c c}
%\hline
\subf{\includegraphics[width=51mm]{figs/FrozenConceptAnalysis/AllPipelines/FrozenConceptAllComparePipeline_dp_p_p_eta_0 - 1.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=51mm]{figs/FrozenConceptAnalysis/AllPipelines/FrozenConceptAllComparePipeline_dp_p_p_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=51mm]{figs/FrozenConceptAnalysis/AllPipelines/FrozenConceptAllComparePipeline_dp_p_p_eta_2.5 - 3.5.pdf}}
    {}

\\
%\hline

\end{tabular}
\caption{\cris{This is a place-holder; will be updated} Momentum resolution of different pipelines corresponding to different possible combinations of technology optimized with AI. %It is shown that any given combination of technology (pipeline) can optimized using the developed framework. 
Pipeline-IV was eventually chosen as the new reference design for the inner barrels. It should be noted that the AI-optimized configurations outperformed the original designs in all $\eta$ bins. Specifically, the optimized pipelines meet the YR PWG requirement in the region $1.0 \leq \eta < 2.5$. }\label{fig:Phase-I_Pipelines}
\end{figure*}

As a result of the Phase-I AI-assisted optimization, pipeline-IV (made by 2 vtx (ITS3-MAPS), 2 sagitta (ITS3-MAPS), 2 outer ($\mu$Rwell)) was chosen by ECCE (after discussing the results with the DWG and the PWG, see Fig.~\ref{fig:pipeline_workflow}) as the new inner tracker barrel design.
Detailed simulation of the PID and TOF detectors were made after Phase-I optimization.
At this point, the arrangement of disks in the electron-going and hadron-going directions was no more symmetric. A realistic support structure has been also implemented, along with new constraints, updated simulations of the detector system and more realistic support structures. The pipeline-IV has been selected as the new reference for the next phase (Phase-I I) in this continued optimization process.

\end{comment}



%\begin{itemize}
    %\item Out of the pipelines that were optimized, 2 pipelines were potentially chosen as they readily satisfy the PWG requirement in the central region. Also, All the pipelines improve the momentum resolution in the transition region. 
    %\item Pipeline-4 \Big [ 2 vtx (ITS3-MAPS) + 2 sagitta (ITS3-MAPS) + 2 outer ($\mu$Rwell) \Big ] was chosen by the proto-collaboration since it was chosen as the new inner tracker barrel design for ECCE.  
    
    %\item The important role of AI is to steer the decision towards choosing a pipeline. AI had assisted in choosing the appropriate technology for the inner tracking barrels (Pipeline-4). This choice of technology was not only made by simply swapping the barrel layers with different combinations but an extensive optimization was done to show that chosen pipeline can be optimized the most and also at the same time realisable by the DWG. 
    %\item Pipeline-4 is now the new reference design for the inner barrels. Detailed simulation of the PID and TOF detectors were made by end of Phase-I optimization. The arrangement of disks in the electron-going and hadron-going directions were no more symmetric. There were implementation of realistic support structure. Therefore with new constraints and updated simulations of detector system and more realistic support structures and pipeline-4 as the new updated reference design next phase (Phase-II) of optimizations continued.
   
%\end{itemize}


%--- end Karthik comment 
%%%%% End of Phase-I results %%%%%%%


%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Design Performance --- Non-projective vs Projective:} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Results shown in this paragraph have been obtained during the optimization Phase II. 


\begin{comment}

Fig.~\ref{fig:Phase-II_Momentum_res} shows the momentum resolution for the non-projective ECCE tracker reference design and the ongoing project R\&D on the projective mechanical structure for the ECCE tracker design in bins of pseudo-rapidity.
Similarly Fig.~\ref{fig:Phase-II_dth_res} shows the angular resolution while Fig.~\ref{fig:Phase-II_KF_eff} shows the Kalman filter efficiency as defined in Eq.~\eqref{eq:objective_KF}.
\end{comment}

%\cris{Move Figures \ref{fig:Phase-II_Momentum_res}, \ref{fig:Phase-II_dth_res}, \ref{fig:Phase-II_KF_eff}, \ref{fig:Phase-II_dph_res}, \ref{fig:Phase-II_recon_eff} in Appendix.}





\begin{comment}
%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Validation}\label{subsec:validation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Validation is performed by looking at figures of merit that are not used in the optimization process. Also in Sec.~\ref{subsec:physics_analysis} we perform a physics analysis with SIDIS events to further consolidate our conclusions.
We show here as an example in Fig.~\ref{fig:Phase-II_dph_res} and Fig.~\ref{fig:Phase-II_recon_eff} the azimuthal angular resolution and the reconstruction efficiency obtained for both the non-projective and the projective ECCE tracker.
The azimuthal resolution looks consistent within the uncertainty for the two designs, while the reconstruction efficiency looks in general better for the projective design, particularly in the 1 $<$ $|\eta|$ $<$ 1.5 region where the non-projective has a larger dead area that affect the reconstruction of tracks.
\end{comment}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph{validation of Phase-II projective}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sec. 3 on Simulations 


%The ECCE tracking system strategically deploys two novel technologies: 
%
%Furthermore, as shown in Figure~\ref{fig:tracking}, the tracking system is tightly integrated with the PID detectors. 
%In particular, the AC-LGAD based Time of Flight (ToF) detectors will also provide precision space-time measurements on the track. 


%%All repositories are documented here \cite{ecce_eic_repo}.

%%The concept of Node Tree is at the center of the Fun4All software framework \cite{fun4all_doc}, in that this is how data are organized. Data object are stored in DST Tree. The user can utilize C++ based analysis modules to access them, perform analysis and save result in analysis NTuple and/or histograms for final plotting. User usually need to compile the analysis module, run it as part of fun4all reconstruction macro, and plot based on the output ROOT file. The structure of the Fun4All framework is represented in Fig.~\ref{fig:Fun4All_Workflow}.
%A more detailed description of the ECCE Software documentation can be found in the following documentation \cite{ecce_sw_doc}.



\begin{comment}
\begin{figure*}[!ht]
\centering
    \includegraphics[width=0.49\textwidth]{figs/IP6-1.5T-Starting-Setup-11142021-EEMCAL-eta3-tracking2.jpg}
    \includegraphics[width=0.49\textwidth]{figs/Oct-Concept39.png}
    \caption{tracking system of ECCE in mechanical model (left) and Geant4 simulation (right). The tracking system is tightly integrated with the PID detectors which is also shown on the right. Support and cabling for the these detectors was implemented (copper-colored cylinder-cone) to count for its material and acceptance effects.}
    \label{fig:tracking}
\end{figure*}
\end{comment}


%
%For each of the sub-detector described in this document, the dimensions of the detectors can be parametrized based on constraints. 



\begin{comment}
\begin{figure}[!]
    \centering
    %\includegraphics[scale = 0.8]{figs/ProjectionConceptAnalysis/AllinOne.pdf}
    \includegraphics[width=0.45\textwidth]{figs/TechNote_Tracking_GAUSS.pdf}
    \caption{
    \textbf{Momentum resolution for the ECCE tracker reference design and the projective design (ongoing R\&D):} The $\Delta p /p$ are extracted with single-gaussian (SG) fits (circles) to be consistent with the YR PWG and compared to double-gaussian (DG) fits (triangles). DG (see Eq.~\eqref{eq:DG}) is used in the AI-assisted pipelines as it provides more stable fits. DG results are systematically larger than the SG ones as they capture more realistic distributions (see Fig.~\ref{fig:fit_results}). 
    This effect is larger in $1<|\eta|<1.5$ for the non-projective design (blue points) since more material is traversed by the tracks; the same effect is moderately present also in $0.5<|\eta|<1$ for the same reason. 
    In the same bins, the ongoing R\&D design shows a significant reduction of the impact of the readout and services and SG (red circle) and DG (red triangles) are close to each other.  
    DG points are systematically large in $3<\eta<3.5$ and in $-3.5<\eta<3.0$, and this corresponds to edge effects at large $|\eta|$ values close to the inner radii of the disks in the endcaps.  
    In the region $-1<\eta<3.0$ $\Delta p/p$ is consistent with the YR physics requirements with SG. Note that physics in the backward region relies on the EM calorimeter also, and in the proposal it has been demonstrated that larger resolutions are acceptable.  
    \label{fig:Phase-II_Momentum_res}
    }
\end{figure}


\begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ProjectionConceptAnalysis/CompareAll_dth.pdf}
    \caption{\tetxbf{Angular resolution ($d\theta$) for ECCE projective geometry and ECCE simulation:} The resolution shows an improvement in the transition region between $1.0 < |\eta| < 1.5$. These plots have been produced using double-gaussian fits.
    \label{fig:Phase-II_dth_res}
    }
\end{figure}

\begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ProjectionConceptAnalysis/TechNote_KF_Efficiency.pdf}
    \caption{\tetxbf{KF Efficiency for ECCE projective geometry and ECCE simulation:} Reconstruction efficiency shows an improvement in the transition region between $1.0 < |\eta| < 1.5$. There is a significant drop in the transition region caused due to multiple scattering of the support structure. }
    \label{fig:Phase-II_KF_eff}
\end{figure}
\end{comment}




\begin{comment}
\begin{table}[!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{M{2.5cm}|M{3.cm}|M{3.cm}|M{3.5cm}}
        \hline
        & \textbf{design pars} &  \textbf{objectives}\\
        \hline
        \hline
           %\textbf{\#} &  4(11) &  3 (4) &  4(5) %\\
        %\hline
           \textbf{ECCE tracker design (non-projective)} & \small{
           %(Phase-I symmetric design) 5 disks $z$-location (hadron endcap) and 6 barrel layers radii;
           5 disks $z$ (hadron endcap) and 4 disks $z$ (electron end cap) location,  2 $\mu$Rwell layers Radius} & \small{momentum resolution; angular resolution; Kalman filter efficiency; (pointing resolution)}
            \\
        \hline
        \hline
           \textbf{ECCE ongoing R\&D design (projective)} & \small{Angle Tracking Support ($\theta$), 2 TTL $z$-location, 1 uRwell-1 Radius, 3 FST disks, 2 EST disks (9 parameters);} & \small{momentum resolution; angular resolution; Kalman filter efficiency; angular resolution at dRICH; (pointing resolution)}
           & \small{(i) FST/EST Disks $(R_{Max}-R_{Min})\%(30.0 \ mm)=0$; (ii) FST/EST Disks $(R_{Max}-R_{Min})\%(17.8 \ mm)=0$; (iii) FST/EST $z_{n+1} - z_{n} \geq 10$; (iv) Length of vertex support structure $\leq$ 30 cm; (v) distance between any 2 $\mu$Rwell barrel layers have to be $\geq$ 5 cm } 
           %\cris{larger! It was smaller...} 
           \\
        \hline
        \hline
        
    \end{tabular}
    } 
    \caption{ \textbf{Dimensionality of the optimization pipelines:} 
    non-projective design and objective space. Following Eq.~\eqref{eq:moo}, constraints are also included. For each category, a description has been added.  Values in parentheses are the largest ones utilized in the optimization pipelines.
    The Phase-II optimization for non-projective design had less number of parameters to optimize due to the fixed support cone structure.  Notice that two additional constraints are implicitly taken into account, that is: (i) the inner radii of the disks in the endcap and the inner vertex layer in the barrel have to be compatible with the beam envelope dimensions; (ii) the barrel layers lengths and the outer radii of the disks have to be compatible with an Al-shell support structure provided by the LBNL design \cite{arrington2021eic}. Conditions (i) and (ii) are provided by internal parametrization and reflected in the Geant4 design. Potential overlaps among modules are checked before and during the optimization. }
    \label{tab:dimensionality}
\end{table}
\end{comment}




\begin{comment}
The Electron-Ion Collider (EIC) is a cutting-edge accelerator facility proposed to study the nature of the ``glue'' that binds the building blocks of the visible matter in the universe. The proposed experiment will be realized at Brookhaven National Laboratory in approximately 10 years from now, with the detector design and R\&D currently ongoing. 
%
Noticeably EIC can be one of the first facilities to leverage on Artificial Intelligence (AI) during the design and R\&D phases. Optimizing the design of its tracker is of crucial importance for the EIC Comprehensive Chromodynamics Experiment (ECCE), a consortium that is proposing a detector design based on a 1.5T solenoid. The optimization is an essential part of the design and R\&D and ECCE includes in its structure a working group dedicated to AI-based applications for the EIC detector. 
%
In this note we describe a comprehensive study in detector design of large-scale experiments using AI that has been accomplished during the detector proposal. This work required a complex parametrization of the simulated detector system. % simulated with the Fun4All framework.  
%
Our approach deals with an optimization problem in a multidimensional design space driven by multiple objectives that encode the detector performance, while satisfying several mechanical constraints. 
%
We describe our strategy and show results obtained for the ECCE tracking system. 
The AI-assisted design is agnostic to the simulation framework and can be extended after the detector proposal to other sub-detectors or system of sub-detectors to optimize the performance of the EIC detector.  
\end{comment}



\begin{comment}
\begin{table}[!]
    \centering
    %\resizebox{\columnwidth}{!}{
    \begin{adjustbox}{width=\columnwidth}
    %\begin{tabular}{| c | c | c |}
    \begin{tabular}{|M{5.cm}|M{3.cm}|M{3.5cm}|}
        \hline 
        \rowcolor{blue!15}\multicolumn{3}{|c|}{  \textbf{ECCE design (non-projective)}}\\
        \hline
        \textbf{Design Parameter} & \textbf{Reference value} & \textbf{Range} \\
        \hline
        $\mu$RWELL 1 (Inner) ($r$) Radius & 44.2 cm & [17.0, 51.0 cm] \\
        \hline
        $\mu$RWELL 2 (Inner) ($r$) Radius & 47.4 cm & [18.0, 51.0 cm] \\
        \hline
        EST 4 $z$ position &  -107.1 cm & [-110.0, -50.0 cm] \\
        \hline
        EST 3 $z$ position &  -80.0 cm & [-110.0, -40.0 cm] \\
        \hline
        EST 2 $z$ position &  -57.5 cm & [-80.0, -30.0 cm] \\
        \hline
        EST 1 $z$ position &  -35.0 cm & [-50.0, -20.0 cm] \\
        \hline
        FST 1 $z$ position & 35.0 cm & [20.0, 50.0 cm] \\
        \hline 
        FST 2 $z$ position & 57.5 cm & [30.0, 80.0 cm] \\
        \hline
        FST 3 $z$ position & 80.0 cm & [40.0, 110.0 cm] \\
        \hline
        FST 4 $z$ position & 115.0 cm & [50.0, 125.0 cm] \\
        \hline
        FST 5 $z$ position & 125.0 cm & [60.0, 125.0 cm] \\
        \hline
        \rowcolor{blue!15}\multicolumn{3}{|c|}{  \textbf{ECCE ongoing R\&D (projective)}}\\
        \hline
        \textbf{Design Parameter} & \textbf{Reference value} & \textbf{Range} \\
        \hline
        Angle (Support Cone) & 25.5 $\degree$ & [25.0$\degree$, 30.0$\degree$] \\
        \hline
        $\mu$RWELL 1 (Inner) Radius & 33.12 cm & [25.0, 45.0 cm] \\
        \hline
        ETTL $z$ position & -169.0 cm & [-171.0, -161.0 cm] \\
        \hline
        EST 2 $z$ position &  -80.05 cm & [45, 100 cm] \\
        \hline
        EST 1 $z$ position & -33.2 cm & [35, 50 cm] \\
        \hline
        FST 1 $z$ position & 33.2 cm & [35, 50 cm] \\
        \hline 
        FST 2 $z$ position & 79.85 cm & [45, 100 cm] \\
        \hline
        FST 5 $z$ position & 144 cm & [100, 150 cm] \\
        \hline
        FTTL $z$ postion & 182 & [156, 183 cm] \\
        \hline
        
    \end{tabular}
    \end{adjustbox}
    \caption{\textbf{Ranges of the design parameters:}  the table summarises the design points that are optimized for the non-projective and the projective case. The optimization range is also given for each parameter. The parameters corresponding to the non-projective case were optimized sequentially over at least three iterations, with each iteration having a set of parameters fixed. For instance, the EST/FST disks were optimized during the first iteration assuming symmetric design, and for the subsequent iterations the EST disks were optimized further in the electron endcap region.  
    %The other geometric parameter for each of the detector systems are calculated based on the parametrization discussed above. 
    Along with the design parameters the design comes with geometrical constraints too. 
    These are implemented as strong and soft constraints in the Table \ref{tab:constraints}. 
    \label{tab:ranges}
    }
\end{table}
\end{comment}


\begin{comment}
A thorough comparison between the non-projective ECCE simulation and the ongoing R\&D was carried out to optimize the support structure through a projective design.  
%
Fig.~\ref{fig:Phase-II_Momentum_res} shows a study of the obtained  momentum resolution 
%for the non-projective ECCE tracker reference design and the ongoing project R\&D on the projective mechanical structure for the ECCE tracker design 
in bins of pseudorapidity.
Similarly Fig.~\ref{fig:Phase-II_dth_res} shows the angular resolution while Fig.~\ref{fig:Phase-II_KF_eff} shows the Kalman filter efficiency as defined in Eq.~\eqref{eq:objective_KF}.
\end{comment}



\begin{comment}
Such improvement in resolution is the result of a continued multi-objective optimization process as described in Sec. \ref{sec:analysis} and summarized in Fig. \ref{fig:continued_optimization}, where the momentum resolution 
obtained during phase-I optimization using a preliminary detector concept is compared to both the non-projective and the projective R\&D designs which are instead derived from fully developed simulations in phase-II optimization.
\end{comment}


\begin{comment}
\begin{figure*}[!]
    \centering
    \includegraphics[width=0.23\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_0 - 1.pdf}
    \includegraphics[width=0.23\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_1 - 1.5.pdf}
    \includegraphics[width=0.23\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_1.5 - 2.5.pdf}
    \includegraphics[width=0.23\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_2.5 - 3.5.pdf}
    \caption{\textbf{Evolution of momentum resolution driven by the continued MOO:} Momentum resolutions in four bins of $\eta$. From left to right, respectively: $|\eta|<$ 1.0 corresponding to the barrel, 1.0 $|\leq \eta<|$ 1.5 corresponding to the transition region, and 1.5 $\leq |\eta| <$ 2.5 and 2.5 $\leq \eta <$ 3.5 corresponding to the two end-caps. Black points represent the first simulation campaign, and a preliminary detector concept in phase-I optimization which did not have a developed support structure; blue points represent the fully developed simulations for the final ECCE detector proposal concept; red points the ongoing R\&D for the optimization of the support structure. Compared to black, there is an improvement in performance in all $\eta$ bins with the exception of the transition region, an artifact that depends on the fact that black points do not include a realistic simulation of the material budget in the transition region. In the transition region, it can be also appreciate the improvement provided by the projective design. %\cris{polish text; reference in the document; move figures and reduce blank spaces}
    }
    \label{fig:continued_optimization}
\end{figure*}
\end{comment}
